EIFFeL: Ensuring Integrity for Federated Learning

Federated learning (FL) enables clients to collaborate with a server to train a machine learning model. To ensure privacy, the server performs secure aggregation of updates from the clients. Unfortunately, this prevents verification of the well-formedness (integrity) of the updates as the updates are masked. Consequently, malformed updates designed to poison the model can be injected without detection. In this paper, we formalize the problem of ensuring \textit{both} update privacy and integrity in FL and present a new system, \textsf{EIFFeL}, that enables secure aggregation of \textit{verified} updates. \textsf{EIFFeL} is a general framework that can enforce \textit{arbitrary} integrity checks and remove malformed updates from the aggregate, without violating privacy. Our empirical evaluation demonstrates the practicality of \textsf{EIFFeL}. For instance, with $100$ clients and $10\%$ poisoning, \textsf{EIFFeL} can train an MNIST classification model to the same accuracy as that of a non-poisoned federated learner in just $2.4s$ per iteration.

==> Copy/Abstract+intro.tex <==
Federated learning enables a centralized server to train machine-learning models on data provided by clients, while preserving the privacy of that data.A major downside of such centralized federated learning is that the server cannot verify the integrity of the data ingested into the learner.This allows malicious clients to stage data-poisoning attacks, and it makes the learner susceptible to Byzantine errors.This paper presents a new protocol, called \name, that allows the server to implement an arbitrary function that verifies the integrity of input data in a privacy-preserving way.\name~uses this function to filter out invalid data in the secure aggregation performed by the federated learner, without the server learning how the data was filtered.The computational and communication overhead of \name is limited.
Our experimental evaluation demonstrates that \name enables the implementation of sophisticated data-integrity checks in real-world federated learners.



The goal of centralized federated learning is for a server to learn the parameters of a machine-learning model based on data provided by (a large number of) clients, without learning the contents of that data~\cite{mcmahan2017communication}.
Many protocols for federated learning~\cite{bonawitz2017practical,konecny2015federated,mcmahan2017communication} do so in a secure and privacy-preserving way by performing secure aggregation of parameter gradients: each client shares a ciphertext of its own gradient with the server, and the server sums the encrypted gradients, decrypts the resulting aggregate gradient, and uses the result to update the model.
If the number of clients involved in the aggregation is sufficiently large, this leaks hardly any information about an individual client's gradient, hence preserving the privacy of that data.
The amount of information leakage can optionally be bounded via a differentially private release mechanism~\cite{mcmahan2017learning}.

A major disadvantage of secure aggregation is that the server has no visibility into the parameter gradients ingested into the federated learner. 
This makes it impossible to detect malicious clients that are staging data-poisoning attacks~\cite{bagdasaryan2018backdoor,bhagoji2019analyzing,kairouz2019advances} against the federated learner.
In such attacks, one or more (colluding) adversarial clients ingest inputs into the learner that are specifically crafted to increase the error of the model~\cite{biggio2021poisoning,mei2015teaching} or to create targeted back-doors in that model that can be exploited later~\cite{chen2017targeted}.
Even if all clients involved in the federated learner can be trusted, the server's inability to ensure the integrity of the inputs may be problematic when inadvertent errors occur, as gradient-based learners are not robust to Byzantine errors~\cite{blanchard2017machine,chen2017distributed,chen2018draco,xie2018generalized}.

This observation naturally leads to the research question we address in this paper: \emph{How can a federated learner efficiently verify the integrity of clients' data without violating the privacy of data?}
We develop a new protocol for federated learning, called \name, that uses secret-shared non-interactive proofs (SNIPs;~\cite{corrigan2017prio}) to evaluate a verification function on the data to ensure its integrity, and that removes invalid data from the secure aggregation.
In the \name{} protocol, the server does not learn anything about the data: invalid data is removed from the aggregation results unbeknownst to the server.
In contrast to prior work~\cite{burkhalter2021rofl}, our verification function can be an arbitrary function that can be implemented by an arithmetic circuit that operates on a single parameter-gradient vector.
This allows \name{} to implement sophisticated procedures to ensure robustness of the learner~\cite{sun2019backdoor,xie2019zeno,xie2020zeno}.
Our protocol requires only a small additional number of rounds of communication between a client and the server compared to vanilla secure aggregation.
The amount of additional communication required is linear in the size of the arithmetic circuit.
We perform experiments with an implementation of \name, which suggest that its computational and communication overhead is sufficiently low for it to form the basis of real-world federated learners~\cite{bonawitz2017practical} that ensure data integrity in a privacy-preserving way.

